AI-Enabled Operations at Fermi Complex: Multivariate Time Series Prediction for Outage Prediction and Diagnosis

The Main Control Room of the Fermilab accelerator complex continuously gathers extensive time-series data from thousands of sensors monitoring the beam. However, unplanned events such as trips or voltage fluctuations often result in beam outages, causing operational downtime. This downtime not only consumes operator effort in diagnosing and addressing the issue but also leads to unnecessary energy consumption by idle machines awaiting beam restoration. The current threshold-based alarm system is reactive and faces challenges including frequent false alarms and inconsistent outage-cause labeling. To address these limitations, we propose an AI-enabled framework that leverages predictive analytics and automated labeling. Using data from $2,703$ Linac devices and $80$ operator-labeled outages, we evaluate state-of-the-art deep learning architectures, including recurrent, attention-based, and linear models, for beam outage prediction. Additionally, we assess a Random Forest-based labeling system for providing consistent, confidence-scored outage annotations. Our findings highlight the strengths and weaknesses of these architectures for beam outage prediction and identify critical gaps that must be addressed to fully harness AI for transitioning downtime handling from reactive to predictive, ultimately reducing downtime and improving decision-making in accelerator management.

==> predict_by_n_models.tex <==
\begin{table}[]
    \centering
        \caption{Caption}
    \label{tab:my_label}

    \resizebox{0.4\textwidth}{!}{\begin{tabular}{lrr}
\toprule
 & Either & Both \\
\midrule
KRF1 CS Fault (11) & 0.73 & 0.18 \\
KRF2 CS Fault (30) & 0.27 & 0.50 \\
KRF5 CS Fault (15) & 0.47 & 0.40 \\
LRF Fault (18) & 0.56 & 0.22 \\
Other (3) & 0.33 & 0.67 \\
other (3) & 0.33 & 0.33 \\
\bottomrule
\end{tabular}}
\end{table}

==> sensitivity_analysis.tex <==
\begin{longtable*}[!ht]
	%\setlength{\tabcolsep}{1pt}
	\centering
	\caption{Sensitivity analysis}
	\label{tab:sensitivityAnalysis}
	\begin{threeparttable}[b]
    % \resizebox{\textwidth}{!}{%
		\begin{tabular}{@{}lccccccccc@{}}
			\toprule
			& \textbf{MSE} & \textbf{n\_outages} & \textbf{n\_detected} & \textbf{Time diff.} & \textbf{n\_early} & \textbf{n\_late} & \textbf{False} & \textbf{n\_non}& \textbf{False}  \\
			& \textbf{(Test)} & & & \textbf{(in seconds)} & & & \textbf{Negatives} & \textbf{outages} & \textbf{Positives}\\
			\midrule
                \textbf{LSTM}\\
			    \bfseries Baseline & \bfseries 0.21 & \bfseries 80 & \bfseries 80 & \bfseries -11.16 & \bfseries 75 & \bfseries 5 & \bfseries 0 & \bfseries 31 & \bfseries 9 \\
			    \cmidrule{2-11}
			    $L_b=45$& 0.21 & 80 & 80 & -9.07 & 70 & 10 & 0 & 31 & 6 \\
			$L_b=60$& 0.21 & 80 & 80 & -7.81 & 67 & 13 & 0 & 31 & 5 \\
			$L_b=90$& 0.24 & 80 & 74 & -6.84 & 63 & 11 & 6 & 31 & 5 \\
			\cmidrule{2-11}
			    $G=0$& 0.15 & 80 & 80 & -1.60 & 25 & 55 & 0 & 31 & 2 \\
                $G=15$& 0.18 & 80 & 80 & -9.60 & 68 & 12 & 0 & 31 & 8 \\
			$G=60$& 0.25 & 80 & 80 & -12.31 & 78 & 2 & 0 & 31 & 10 \\
                \cmidrule{2-11}
			    BCEL$^{\dag}$& 17.67 & 80 & 80 & -10.38 & 71 & 9 & 0 & 31 & 9 \\
                MAE$^{\ast}$& 0.22 & 80 & 80 & -10.05 & 72 & 8 & 0 & 31 & 12 \\

                \midrule
                \textbf{Transformer}\\
                \bfseries Baseline & \bfseries 0.21 & \bfseries 80 & \bfseries 79 & \bfseries -9.62 & \bfseries 72 & \bfseries 7 & \bfseries 1 & \bfseries 31 & \bfseries 8 \\
			\cmidrule{2-11}
			    $L_b=45$ & 0.20 & 80 & 79 & -4.74 & 48 & 31 & 1 & 31 & 4 \\
			$L_b=60$ & 0.20 & 80 & 77 & -3.84 & 51 & 26 & 3 & 31 & 2 \\
			$L_b=90$ & 0.23 & 80 & 76 & -3.39 & 49 & 27 & 4 & 31 & 2 \\
			\cmidrule{2-11}
			    $G=0$ & 0.16 & 80 & 79 & -3.61 & 43 & 36 & 1 & 31 & 4 \\
			$G=15$ & 0.17 & 80 & 80 & -6.74 & 62 & 18 & 0 & 31 & 8 \\
			$G=60$ & 0.21 & 80 & 80 & -10.27 & 77 & 3 & 0 & 31 & 6  \\
			\cmidrule{2-11}
			    BCEL$^{\dag}$ & 17.77 & 80 & 80 & -9.40 & 70 & 10 & 0 & 31 & 3 \\
                MAE$^{\ast}$ & 0.24 & 80 & 80 & -10.80 & 75 & 5 & 0 & 31 & 7 \\
                
                \midrule
			\textbf{N-HiTS}\\
                \bfseries Baseline & \bfseries 0.17 & \bfseries 80 & \bfseries 79 & \bfseries -9.34 & \bfseries 71 & \bfseries 8 & \bfseries 1 & \bfseries 31 & \bfseries 10 \\
			\cmidrule{2-11}
			    $L_b=45$ & 0.19 & 80 & 78 & -7.16 & 66 & 12 & 2 & 31 & 6 \\
			$L_b=60$ & 0.19 & 80 & 79 & -8.27 & 71 & 8 & 1 & 31 & 12 \\
			$L_b=90$ & 0.20 & 80 & 75 & -8.86 & 74 & 1 & 5 & 31 & 20 \\
			\cmidrule{2-11}
			    $G=0$ & 0.12 & 80 & 79 & -9.21 & 72 & 7 & 1 & 31 & 19 \\
			$G=15$ & 0.16 & 80 & 79 & -11.86 & 77 & 2 & 1 & 31 & 16 \\
			$G=60$ & 0.20 & 80 & 80 & -11.53 & 79 & 1 & 0 & 31 & 14 \\
			\cmidrule{2-11}
			    BCEL$^{\dag}$ & 193.98 & 80 & 79 & -6.60 & 61 & 18 & 1 & 31 & 2 \\
                MAE$^{\ast}$ & 0.18 & 80 & 80 & -11.43 & 77 & 3 & 0 & 31 & 15 \\
			\bottomrule

            \midrule
			\textbf{N-HiTS}\\
                \bfseries Baseline & \bfseries 0.17 & \bfseries 80 & \bfseries 79 & \bfseries -9.34 & \bfseries 71 & \bfseries 8 & \bfseries 1 & \bfseries 31 & \bfseries 10 \\
			\cmidrule{2-11}
			    $L_b=45$ & 0.19 & 80 & 78 & -7.16 & 66 & 12 & 2 & 31 & 6 \\
			$L_b=60$ & 0.19 & 80 & 79 & -8.27 & 71 & 8 & 1 & 31 & 12 \\
			$L_b=90$ & 0.20 & 80 & 75 & -8.86 & 74 & 1 & 5 & 31 & 20 \\
			\cmidrule{2-11}
			    $G=0$ & 0.12 & 80 & 79 & -9.21 & 72 & 7 & 1 & 31 & 19 \\
			$G=15$ & 0.16 & 80 & 79 & -11.86 & 77 & 2 & 1 & 31 & 16 \\
			$G=60$ & 0.20 & 80 & 80 & -11.53 & 79 & 1 & 0 & 31 & 14 \\
			\cmidrule{2-11}
			    BCEL$^{\dag}$ & 193.98 & 80 & 79 & -6.60 & 61 & 18 & 1 & 31 & 2 \\
                MAE$^{\ast}$ & 0.18 & 80 & 80 & -11.43 & 77 & 3 & 0 & 31 & 15 \\

            \midrule
			\textbf{N-HiTS}\\
                \bfseries Baseline & \bfseries 0.17 & \bfseries 80 & \bfseries 79 & \bfseries -9.34 & \bfseries 71 & \bfseries 8 & \bfseries 1 & \bfseries 31 & \bfseries 10 \\
			\cmidrule{2-11}
			    $L_b=45$ & 0.19 & 80 & 78 & -7.16 & 66 & 12 & 2 & 31 & 6 \\
			$L_b=60$ & 0.19 & 80 & 79 & -8.27 & 71 & 8 & 1 & 31 & 12 \\
			$L_b=90$ & 0.20 & 80 & 75 & -8.86 & 74 & 1 & 5 & 31 & 20 \\
			\cmidrule{2-11}
			    $G=0$ & 0.12 & 80 & 79 & -9.21 & 72 & 7 & 1 & 31 & 19 \\
			$G=15$ & 0.16 & 80 & 79 & -11.86 & 77 & 2 & 1 & 31 & 16 \\
			$G=60$ & 0.20 & 80 & 80 & -11.53 & 79 & 1 & 0 & 31 & 14 \\
			\cmidrule{2-11}
			    BCEL$^{\dag}$ & 193.98 & 80 & 79 & -6.60 & 61 & 18 & 1 & 31 & 2 \\
                MAE$^{\ast}$ & 0.18 & 80 & 80 & -11.43 & 77 & 3 & 0 & 31 & 15 \\
			\bottomrule

            \midrule
			\textbf{N-HiTS}\\
                \bfseries Baseline & \bfseries 0.17 & \bfseries 80 & \bfseries 79 & \bfseries -9.34 & \bfseries 71 & \bfseries 8 & \bfseries 1 & \bfseries 31 & \bfseries 10 \\
			\cmidrule{2-11}
			    $L_b=45$ & 0.19 & 80 & 78 & -7.16 & 66 & 12 & 2 & 31 & 6 \\
			$L_b=60$ & 0.19 & 80 & 79 & -8.27 & 71 & 8 & 1 & 31 & 12 \\
			$L_b=90$ & 0.20 & 80 & 75 & -8.86 & 74 & 1 & 5 & 31 & 20 \\
			\cmidrule{2-11}
			    $G=0$ & 0.12 & 80 & 79 & -9.21 & 72 & 7 & 1 & 31 & 19 \\
			$G=15$ & 0.16 & 80 & 79 & -11.86 & 77 & 2 & 1 & 31 & 16 \\
			$G=60$ & 0.20 & 80 & 80 & -11.53 & 79 & 1 & 0 & 31 & 14 \\
			\cmidrule{2-11}
			    BCEL$^{\dag}$ & 193.98 & 80 & 79 & -6.60 & 61 & 18 & 1 & 31 & 2 \\
                MAE$^{\ast}$ & 0.18 & 80 & 80 & -11.43 & 77 & 3 & 0 & 31 & 15 \\
			\bottomrule
			\bottomrule
		\end{tabular}%}
    % \footnotesize
    \begin{tablenotes}
        \item[$\dag$] BCEL: Binary Cross Entropy with Logits Loss \\(\texttt{torch.nn.BCEWithLogitsLoss}) 
        \item[$\ast$] MAE: Mean Absolute Error (\texttt{torch.nn.L1Loss})
    \end{tablenotes}
    \end{threeparttable}
\end{longtable*}
